Scaling Stick-Breaking Attention: An Efficient Implementation and In-depth Study

The self-attention mechanism traditionally relies on the softmax operator, necessitating positional embeddings like RoPE, or position biases to account for token order. But current methods using still face length generalisation challenges. We investigate an alternative attention mechanism based on the stick-breaking process in larger scale settings. The method works as follows: For each token before the current, we determine a break point, which represents the proportion of the stick, the weight of the attention, to allocate to the current token. We repeat this on the remaining stick, until all tokens are allocated a weight, resulting in a sequence of attention weights. This process naturally incorporates recency bias, which has linguistic motivations for grammar parsing. We study the implications of replacing the conventional softmax-based attention mechanism with stick-breaking attention. We then discuss implementation of numerically stable stick-breaking attention and adapt Flash Attention to accommodate this mechanism. When used as a drop-in replacement for current softmax+RoPE attention systems, we find that stick-breaking attention performs competitively with current methods on length generalisation and downstream tasks. Stick-breaking also performs well at length generalisation, allowing a model trained with $2^{11}$ context window to perform well at $2^{14}$ with perplexity improvements.

==> scratch.tex <==

\begin{table*}[t!]
\caption{}
\label{tab:main_results}
\centering
\small
\addtolength{\tabcolsep}{-2.5pt}    
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model}  & \textbf{Wiki.}  &  \textbf{LMB.} &  \textbf{LMB.} & \textbf{PIQA} &    \textbf{Hella.} & \textbf{Wino.} & \textbf{ARC-e} &  \textbf{ARC-c} \\
 & ppl $\downarrow$  &  ppl $\downarrow$  &  acc $\uparrow$  & acc $\uparrow$ &   acc\_norm $\uparrow$  & acc $\uparrow$  & acc $\uparrow$ & acc\_norm $\uparrow$ \\
\midrule
\small{\textit{Random baseline}} & - & - & - & 25.0 & 25.0 &	50.0 & 25.0	& 25.0 \\
% \cmidrule(l){1-1} \cmidrule(l){2-3} \cmidrule(l){4-9}
\midrule
\multicolumn{9}{l}{\small{\textit{340M parameters, 15B training tokens}}}  \\[.3em]
\hspace{2mm} Transformer++ & \text{28.39} & 42.69 & \text{31.0} & 63.3 & 34.0 &	50.4 & 44.5	& \text{24.2} \\
\hspace{2mm}  RetNet  & 32.33 &	49.19 &	28.6 &	63.5 & 33.5 &	\text{52.5} &	44.5 &	23.4 \\
\hspace{2mm}  Mamba  & \text{28.39} & \text{39.66} & 30.6 & \text{65.0} & \text{35.4} & 50.1 & \text{46.3} & 23.6  \\ 
\hspace{2mm}  GLA Transformer  & 28.65 &	43.35 &	30.3 &	64.8  & 34.5 & 51.4  & 45.1	 & 22.7 \\
%\cmidrule(l){1-1} \cmidrule(l){2-3} \cmidrule(l){4-9}
\cmidrule(l){1-9}
\multicolumn{9}{l}{\small{\textit{1.3B parameters, 100B training tokens}}} \\[.3em]
\hspace{2mm}  Transformer++ & \text{16.85} & \text{13.44} &  \text{48.9} & 70.8 & 49.6 & 53.6 & 56.0 & 26.5 \\
\hspace{2mm}  RetNet  & 18.64 & 17.27 & 43.3 & 70.0 & 47.3 & 52.5 & 54.8 & 25.6 \\
\hspace{2mm}  Mamba  & 17.06 & 13.89 & 46.2 & \text{72.2} &  40.1 & \text{54.1} &  \text{59.0} &	\text{28.2} \\
\hspace{2mm} GLA Transformer & 17.22 & 14.47 & 46.9 & 71.8 & \text{49.8} & 53.9 & 57.2 & 26.6   \\

\bottomrule
\end{tabular}
\addtolength{\tabcolsep}{2.5pt}    
\centering

\end{table*}


\begin{figure}
  \centering
\def\FileName{figures/sweep_diagram.png}
\newsavebox\IBox
\savebox\IBox{\includegraphics[scale=1.0]{\FileName}}
\newcommand{\figscale}{0.2}
\begin{subfigure}{0.24\linewidth}
    \includegraphics[scale=\figscale,viewport=0 0 {0.241\wd\IBox} {\ht\IBox},clip]{\FileName}
    \caption{Forward pass}\label{fig:forward}
\end{subfigure}
\begin{subfigure}{0.49\linewidth}
\includegraphics[scale=\figscale,viewport={0.241\wd\IBox} 0 {0.48\wd\IBox} {\ht\IBox},clip]{\FileName} \includegraphics[scale=\figscale,viewport={0.48\wd\IBox} 0 {0.75\wd\IBox} {\ht\IBox},clip]{\FileName}
\caption{2-phase backward pass}\label{fig:backward}
\end{subfigure}
\begin{subfigure}{0.24\linewidth}
\includegraphics[scale=\figscale,viewport={0.75\wd\IBox} 0 {\wd\IBox} {\ht\IBox},clip]{\FileName}
\caption{Block Skipping}
\end{subfigure}
\caption{Thread tile assignments for a given attention head and a sequence. Tiles coloured the same are processed by the same thread.
For stick-breaking, the forward pass has to be computed from right-to-left, while the backward pass is computed in two-phases: left-to-right for $\nabla\mQ$, and top-to-bottom for $\nabla\mV,\nabla\mK$. 
Uncoloured tiles are not computed: upper right tiles are not used in causal language modelling, and in the case of block skipping, some blocks can be skipped if all entries have summed to 1.
The accumulated values $\textcolor{darkred}{\va}, \textcolor{blue}{\vb}$ are highlighted at the borders for a visual representation of where they are used.}
\end{figure}


We  modify the Triton implementation of Flash Attention for accelerating the stick-breaking attention.
In theory, the memory complexity of implementing stick-breaking attention would be similar to that of Flash Attention, $O(L)$.
Due to the limitations of Triton, we borrow from \citet{dao2023flashattention} and use a two-phased backward pass: the first phase accumulating gradients for $\mQ$ , and the second phase accumulates gradients for $\mK, \mV$.
Due to the intermediate accumulated values $\textcolor{darkred}{\va}, \textcolor{blue}{\vb}$,  our implementation results in a $O(L^2)$ memory complexity.
However, the constant factor in the quadratic complexity here is inverse of the predetermined block size $d_\mathrm{block}$: larger block sizes reduces the memory allocation.
In our implementation, $d_\mathrm{block} = 64$.
Algorithms \ref{alg:forward} details the forward pass (illustrated in Figure \ref{fig:forward}), and Algorithm \ref{alg:backward} details the backward pass (illustrated in Figure \ref{fig:backward}).
\begin{figure}
    \centering
\vspace{-2em}
\begin{minipage}[t]{0.49\textwidth}
\begin{algorithm}[H]
\small
\begin{algorithmic}
   \caption{\textsc{Backward-$\vq$} thread $i$} \label{alg:backwardq}
   \STATE $\textcolor{blue}{\vb} \leftarrow \mathbf{0}, \mO \leftarrow \mathbf{0}$
    \STATE $\nabla\mO \leftarrow $ load block $i$ of $\nabla\mO$
    \STATE $\mQ \leftarrow $ load block $i$ of $\mQ$
    \FOR{$k$ in $1 \hdots i$}
        \STATE $\mK \leftarrow $ load block $k$ of $\mK$
        \STATE $\mV \leftarrow $ load block $k$ of $\mV$
        \STATE $\textcolor{darkred}{\va} \leftarrow$ load block $(i, k)$ of $\textcolor{darkred}{\mM}$
        \STATE \textcolor{orange}{\textbf{Do } \circled{1}}
        \STATE $\nabla \tilde{\mA} \leftarrow \mA \odot ( \nabla\mO \mV^\top)$
        \STATE ${\nabla \tilde{\mA}}_\mathrm{cs} \leftarrow \mathrm{cumsum}_{\rightarrow}\nabla \tilde{\mA}  $
        \STATE $\nabla \mZ \leftarrow \nabla \tilde{\mA}  - (1 - \exp(\mL)) \odot \left({\nabla \tilde{\mA}}_\mathrm{cs} +  \textcolor{blue}{\vb} \right) $
        \STATE $\textcolor{blue}{\vb} \leftarrow \textcolor{blue}{\vb}     + \sum_{\rightarrow} \nabla \tilde{\mA}$ 
        \STATE $\textcolor{blue}{\vb} \rightarrow$ store block $(i, k)$ of $\textcolor{blue}{\mN}$
        \STATE $\nabla\mQ \leftarrow \nabla\mQ + \nabla\mZ \mK^\top $
    \ENDFOR
    \STATE $\nabla\mQ  \rightarrow$ store block $i$ of $\nabla\mQ $
    \STATE
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
\begin{algorithm}[H]
\small
\begin{algorithmic}
   \caption{\textsc{Backward-$\vv$,$\vk$} thread $j$} \label{alg:backwardkv}
    \STATE $\nabla\mK \leftarrow \mathbf{0},\nabla\mV \leftarrow \mathbf{0}$
    \STATE $\mK \leftarrow $ load block $j$ of $\vk$
    \STATE $\mV \leftarrow $ load block $j$ of $\vv$
    \FOR{$k$ in $j \hdots J$}
        \STATE $\mQ \leftarrow $ load block $k$ of $\vq$
        \STATE $\nabla\mO \leftarrow $ load block $k$ of $\nabla\vo$
        \STATE $\textcolor{darkred}{\va} \leftarrow$ load block $(k, j)$ of $\textcolor{darkred}{\mM}$
        \STATE $\textcolor{blue}{\vb} \leftarrow$ load block $(k, j)$ of $\textcolor{blue}{\mN}$
        \STATE \textcolor{orange}{\textbf{Do } \circled{1}}
        \STATE $\nabla \tilde{\mA} \leftarrow \mA \odot ( \nabla\mO \mV^\top)$
        \STATE ${\nabla \tilde{\mA}}_\mathrm{cs} \leftarrow \mathrm{cumsum}_{\rightarrow}\nabla \tilde{\mA}  $
        \STATE $\nabla \mZ \leftarrow \nabla \tilde{\mA}  - (1 - \exp(\mL)) \odot \left({\nabla \tilde{\mA}}_\mathrm{cs} +  \textcolor{blue}{\vb} \right) $
        \STATE $\nabla\mK \leftarrow \nabla\mK + \mA^\top \nabla \mO$
        \STATE $\nabla\mV \leftarrow \nabla\mV + \nabla \mZ^\top \mQ$
        
    \ENDFOR
    \STATE $\nabla\mK  \rightarrow$ store block $j$ of $\nabla\mK $
    \STATE $\nabla\mV  \rightarrow$ store block $j$ of $\nabla\mV $
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}
For stick-breaking, the forward pass has to be computed from right-to-left, while the backward pass is computed in two-phases: left-to-right for $\nabla\mQ$, and top-to-bottom for $\nabla\mV,\nabla\mK$. 
Uncoloured tiles are not computed: upper right tiles are not used in causal language modelling, and in the case of block skipping, some blocks can be skipped if all entries have summed to 1.
The accumulated values $\textcolor{darkred}{\va}, \textcolor{blue}{\vb}$ are highlighted at the borders for a visual representation of where they are used.
\section{Remainder Method}\label{sec:remainder}
We experimented with using remaining attention weight is assigned to the current timestep $\vv_i$, by modifying the output of the attention layer as follows:
\begin{align} 
      \vo_{j} &= \sum_{i=1}^{j-1} \mA_{i,j} \cdot \vv_i + \left(1 - \sum_{i=1}^{j-1} \mA_{i,j}\right) \cdot \vv_j\label{eqn:output}
\end{align}
This way when the attention `does nothing', the value vector for the current time-step is the output for that attention head.
We refer to this modification as `stick-breaking with remainder' (SB w/ rem.).


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.4\linewidth]{figures/length_generalisation_rem.png}
\end{center}
\caption{Length generalisation experiment on 350M model.}
\end{figure}
\begin{table}[h]
    \centering
    \caption{
    Results on the various NLP benchmarks for the 1B and 3B pretrained model.
    `Softmax' benchmark is the standard Softmax + RoPE setting.}\label{tab:1B_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multicolumn{1}{r}{\textbf{Task}} & \textbf{ARC-c} & \textbf{ARC-e} & \textbf{Hella.} & \textbf{OBQA} & \textbf{PIQA} & \textbf{RACE} & \textbf{SciQ} & \textbf{Wino.} & \multirow{2}{*}{\textbf{Avg.}} & \textbf{Wiki.} \\

\multicolumn{1}{c}{} & \multicolumn{4}{c}{\textit{Accuracy (normalised)}} & \multicolumn{4}{c}{\textit{Accuracy}} &  & \multicolumn{1}{c}{\textit{Ppl.}} \\
\cmidrule(r){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10}\cmidrule(l){11-11} 
\multicolumn{11}{l}{~\textit{1B Parameter Models}} \\[.3em]
Softmax & 35.8 & 65.6 & 64.8 & \textbf{38.8} & 75.0 & 36.5 & 90.5 & \textbf{63.4} & 58.8 & 13.8 \\
Stick-breaking & \textbf{37.7} & \textbf{67.6} & \textbf{65.4} & 36.6 & \textbf{76.0} & \textbf{37.4} & \textbf{91.9} & 63.1 & \textbf{59.5} & \textbf{13.4} \\
SB w/ rem. & 35.2 & 66.1 & 64.1 & 38.6 & 75.1 & 36.9 & 90.9 & 62.7 & 58.7 & 13.9 \\
% \cmidrule(r){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10}\cmidrule(l){11-11} 
\bottomrule
\end{tabular}%
}
\end{table}
